Phase transitions in TGFT: a Landau-Ginzburg analysis of Lorentzian quantum geometric models

In the tensorial group field theory (TGFT) approach to quantum gravity, the basic quanta of the theory correspond to discrete building blocks of geometry. It is expected that their collective dynamics gives rise to continuum spacetime at a coarse grained level, via a process involving a phase transition. In this work we show for the first time how phase transitions for realistic TGFT models can be realized using Landau-Ginzburg mean-field theory. More precisely, we consider models generating 4-dimensional Lorentzian triangulations formed by spacelike tetrahedra whose quantum geometry is encoded in non-local degrees of freedom on the non-compact group $\mathrm{SL}(2,\mathbb{C})$ and subject to gauge and simplicity constraints. Further we include $\mathbb{R}$-valued variables which may be interpreted as discretized scalar fields typically employed as a matter reference frame. We apply the Ginzburg criterion finding that fluctuations around the non-vanishing mean-field vacuum remain small at large correlation lengths regardless of the combinatorics of the non-local interaction validating the mean-field theory description of the phase transition. This work represents a first crucial step to understand phase transitions in compelling TGFT models for quantum gravity and paves the way for a more complete analysis via functional renormalization group techniques. Moreover, it supports the recent extraction of effective cosmological dynamics from TGFTs in the context of a mean-field approximation.

==> TGFT meets Landau Ginzburg (2) - Quantum geometric models/fdiagrams.tex <==
\definecolor{jred}{rgb}{0.8,0,0}
\definecolor{jgreen}{rgb}{0,0.7,0}
\definecolor{jblue}{rgb}{0,0,0.8}

\usetikzlibrary{arrows,patterns,shapes,positioning,fit}
\tikzstyle{c} =	[coordinate]
\tikzstyle{vc} = [circle, draw=black, line width=1pt, inner sep=0pt, minimum size=2mm]
\tikzstyle{v} =  [circle, draw=black, line width=.2pt, fill=black, inner sep=0pt, minimum size=1.5mm]
\tikzstyle{vb} =[circle, draw=black, line width=.1pt, fill=jred, inner sep=0pt, minimum size=1mm]
\tikzstyle{vh} =[circle, draw=black, line width=.1pt, fill=jblue, inner sep=0pt, minimum size=1.5mm]
\tikzstyle{vs} =[coordinate]%[circle, draw=black, line width=.1pt, fill=jgreen, inner sep=0pt, minimum size=1mm]
\tikzstyle{e} =	[draw=jred,line width=1pt]
\tikzstyle{eb}= [draw=jgreen,line width=1pt]
\tikzstyle{es}= [dashed, line width=1pt]
\tikzstyle{ev}= [draw=jgreen,line width=1pt]
\tikzstyle{f} = [line width=0.01pt,dotted,fill=blue, fill opacity=.1]
\tikzstyle{cs}= [ellipse, draw=black, line width=.1pt, fill=jred, inner sep=1pt, minimum size=2mm]%[draw=none,fill=jred, fill opacity=.7]

\newcommand{\vertexexstranded}{
\begin{tikzpicture}[x=6ex,y=6ex,baseline={([yshift=-.59ex]current bounding box.center)}] 
    \node [vs]	(12)	at (1,.1)	{};
    \node [vs]	(13)	at (1,0)	{};
    \node [vs]	(14)	at (1,-.1)	{};    
    \node [vs]	(21)	at (.1,1)	{};
    \node [vs]	(24)	at (0,1)	{};
    \node [vs]	(23)	at (-.1,1)	{};    
    \node [vs]	(32)	at (-1,.1)	{};
    \node [vs]	(31)	at (-1,0)	{};
    \node [vs]	(34)	at (-1,-.1)	{};    
    \node [vs]	(41)	at (.1,-1)	{};
    \node [vs]	(42)	at (0,-1)	{};
    \node [vs]	(43)	at (-.1,-1)	{};
    \node [vc, fit=(13) (31)] {};
    \path
    \foreach \i/\j in {14/41,21/12,32/23,43/34}{
    (\i) edge [ev,bend right=40] node [vh] {} (\j)
    }
    \foreach \i/\j in {13/42, 31/24}{
    (\i) edge [ev,bend right=60] node [vh] {} (\j)
    };
    \node [cs,fit=(12) (14)] {};
    \node [cs,fit=(21) (23)] {};
    \node [cs,fit=(32) (34)] {};
    \node [cs,fit=(41) (43)] {};
\end{tikzpicture}
}


\newcommand{\vertexexgraph}{
\begin{tikzpicture}[x=6ex,y=6ex,baseline={([yshift=-.59ex]current bounding box.center)}]    
\scriptsize{
    \node [vb, label=right:${1}$]	(2)	at (0,1)	{};
    \node [vb, label=below:${2}$]	(3)	at (-1,0)	{};
    \node [vb, label=left:${3}$]	(4)	at (0,-1)	{};
    \node [vb,label=above:${4}$]	(1)	at (1,0)	{};
    \node [v, fill=black, minimum size =3mm]   (0) at (0,0)    {};
    \path
    (1) edge [ev] (2)
    (3) edge [ev] (4)
    \foreach \i in {1,2,3,4}{
    (\i) edge [e] (0)
    }
    \foreach \i/\j in {1/4,4/1,2/3,3/2}{
    (\i) edge [ev,bend right=20] node [c] {} (\j)
    };
}
\end{tikzpicture}
}

\newcommand{\vertexexeom}[3]{
\begin{tikzpicture}[x=4ex,y=4ex,baseline={([yshift=-.59ex]current bounding box.center)}]    
\scriptsize{
    \node [vb, label=above:${#1}$]	(2)	at (0,1)	{};
    \node [vb, label=below:${#2}$]	(3)	at (-1,0)	{};
    \node [vb, label=below:${#3}$]	(4)	at (0,-1)	{};
    \node [c]   (a) at (.7,1)   {};
    \node [c]   (b) at (.7,-.8) {};
    \node [c]   (c) at (.7,-1.2){};
    \node [v, fill=black]   (0) at (0,0)    {};
    \path
    (a) edge [ev] (2)
    (3) edge [ev] (4)
    (b) edge [ev] (4)
    (c) edge [ev] (4)
    \foreach \i in {2,3,4}{
    (\i) edge [e] (0)
    }
    \foreach \i/\j in {2/3,3/2}{
    (\i) edge [ev,bend right=20] node [c] {} (\j)
    };
}
\end{tikzpicture}
}

\newcommand{\vertexexvg}{
\begin{tikzpicture}[rotate=45,x=1ex,y=1ex,baseline={([yshift=-.59ex]current bounding box.center)}]    
    \node [vb]	(1)	at (1,0)	{};
    \node [vb]	(2)	at (0,1)	{};
    \node [vb]	(3)	at (-1,0)	{};
    \node [vb]	(4)	at (0,-1)	{};
    \path
    (1) edge [ev] (2)
    (3) edge [ev] (4)
    \foreach \i/\j in {1/4,4/1,2/3,3/2}{
    (\i) edge [ev,bend right=40] node [c] {} (\j)
    };
\end{tikzpicture}
}

\newcommand{\maptadpole}{
\begin{tikzpicture}[x=2ex,y=2ex,baseline={([yshift=-.59ex]current bounding box.center)}]    
    \node [v]	(1)	at (0,0) {};
    \node [c]	(a)	at (-1,0){};
    \node [c]	(b) at (1,0) {};
    \node [c]	(c1)at (0,1) {};
    \path
    (1) edge [e] (a)
    (1) edge [e] (b)
    (1) edge [e, bend right=90] (c1)
    (1) edge [e, bend left=90] (c1);
\end{tikzpicture}
}

\newcommand{\maptadpoledown}{
\begin{tikzpicture}[x=2ex,y=2ex,baseline={([yshift=-.59ex]current bounding box.center)}]    
    \node [v]	(1)	at (0,0) {};
    \node [c]	(a)	at (-1,0){};
    \node [c]	(b) at (1,0) {};
    \node [c]	(c1)at (0,-1) {};
    \path
    (1) edge [e] (a)
    (1) edge [e] (b)
    (1) edge [e, bend right=90] (c1)
    (1) edge [e, bend left=90] (c1);
\end{tikzpicture}
}

\newcommand{\mapsunrise}{
\begin{tikzpicture}[x=2ex,y=2ex,baseline={([yshift=-.59ex]current bounding box.center)}]    
\node [v]	(1)	at (0,0) {};
\node [v]	(2)	at (2,0) {};
\node [c]	(a)	at (-1,0){};
\node [c]	(b) at (3,0) {};
\path
(1) edge [e] (a)
(2) edge [e] (b)
(1) edge [e] (2)
(1) edge [e, bend right=90] (2)
(1) edge [e, bend left=90] (2);
\end{tikzpicture}
}

\newcommand{\mapex}{
\begin{tikzpicture}[x=4ex,y=4ex,baseline={([yshift=-.59ex]current bounding box.center)}]    
    \node [v, label=30:1]	(1)	at (-1.5,0) {};
    \node [v, label=150:2, label=-90:3, label=90:4]	(234)	at (0,0) {};
    \node [v, label=-90:5, label=90:6, label=30:7]	(789)at (1.5,0) {};
    \node [c]	(9)	at (2.25,0) {};
    \path
    (1) edge [e] (234)
    (234) edge [e, bend right=80] (789)
    (234) edge [e, bend left=80] (789)
    (789) edge [e] (9);
\end{tikzpicture}
}

\newcommand{\mapexpq}{
\begin{tikzpicture}[x=3ex,y=3ex,baseline={([yshift=-.59ex]current bounding box.center)}]    
    \node [v]	(1)	at (-1.5,0) {};
    \node [v, label=0:$q$]	(234)	at (0,0) {};
    \node [v, label=30:$p$]	(789)   at (1.5,0) {};
    \node [c]	(9)	at (2.25,0) {};
    \path
    (1) edge [e] (234)
    (234) edge [e, bend right=80] (789)
    (234) edge [e, bend left=80] (789)
    (789) edge [e] (9);
\end{tikzpicture}
}

\newcommand{\mapexstranded}{
\begin{tikzpicture}[x=4ex,y=4ex,baseline={([yshift=-.59ex]current bounding box.center)}]
    \node [vs,label=80:1]	(1a)	at (-2,.05)	{};
    \node [vs]				(1b)	at (-2,-.05)	{};
    \node [c]				(1c)	at (-3,0)	{};
    \node [c]				(1d)	at (-2.5,0)	{};	
    \node [vc, fit=(1a) (1c)] 	{};
    \node [cs,fit=(1a) (1b)] 	{};    
    \node [vs, label=30:2]	(24)	at (-1,.05)	{};
    \node [vs]				(23)	at (-1,-.05)	{};
    \node [c]				(2c)	at (1,-.05)	{};
    \begin{scope}[rotate=120]  
    \node [vs, label=below:3]	(32)	at (-1,.05)	{};
    \node [vs]				(34)	at (-1,-.05)	{};
    \end{scope}
    \begin{scope}[rotate=-120]  
    \node [vs]				(43)	at (-1,.05)	{};
    \node [vs,label=above:4]	(42)	at (-1,-.05)	{};
    \end{scope}
    \node [vc, fit=(23) (2c)] {};
    \node [cs,fit=(24) (23)] {};
    \node [cs,fit=(32) (34)] {};
    \node [cs,fit=(42) (43)] {};
    \path
    \foreach \i/\j in {24/42,32/23,43/34}{
    (\i) edge [ev,bend right=30]  (\j)
    };
    \begin{scope}[xshift=2cm]
    \node [vs, label=0:7]   (89)	at (1,.05)	{};
    \node [vs]				(87)	at (1,-.05)	{};
    \node [c]				(8c)	at (-1,-.05){};
    \begin{scope}[rotate=120]  
    \node [vs, label=80:6]  (97)	at (1,.05)	{};
    \node [vs]				(98)	at (1,-.05)	{};
    \end{scope}
    \begin{scope}[rotate=-120]  
    \node [vs]				(78)	at (1,.05)	{};
    \node [vs,label=-80:5]  (79)	at (1,-.05)	{};
    \end{scope}
    \node [vc, fit=(89) (8c)] {};
    \node [cs,fit=(98) (97)] {};
    \node [cs,fit=(79) (78)] {};
    \path
    \foreach \i/\j in {89/98,97/79,78/87}{
    (\i) edge [ev,bend left=30]  (\j)
    };
    \node [cs,fit=(89) (87)] {};
    \end{scope}    
    \path
    (1a) edge [ev, bend right=70] (1d)
    (1b) edge [ev, bend left=75]	 (1d)
    (1a) edge [ev] (24)
    (1b) edge [ev] (23)
    (42) edge [ev, bend left=60] (98)
    (43) edge [ev, bend left=60] (97)
    (34) edge [ev, bend right=60] (79)
    (32) edge [ev, bend right=60] (78);
\end{tikzpicture}
}
    


    
\newcommand{\mapexvg}{
\begin{tikzpicture}[x=4ex,y=4ex,baseline={([yshift=-.59ex]current bounding box.center)}]        
    \node [v]	(v1)	at (-2.5,0) {};
    \node [c]	(c1)	at (-3,0) 	{};
    \node [v]	(234)	at (0,0) {};
    \node [v]	(789)at (2.6,0) {};
    \node [vb, label=90:1]	(1)	at (-2,0)	{};
    \node [vb, label=90:2]	(2)	at (-1,0)	{};
    \node [vb, label=-90:3]	(3)	at (.6,-1)	{};
    \node [vb, label=90:4]	(4)	at (.6,1)	{};
    \node [vb, label=90:7]	(9)	at (3.6,0)	{};
    \node [vb, label=90:6]	(8)	at (2,1)	{};
    \node [vb, label=-90:5]	(7)	at (2,-1)	{};
    \path
    (v1) edge [e] (1)
    \foreach \i in {2,3,4}{
    (\i) edge [e] (234)
    }
    \foreach \i in {7,8,9}{
    (\i) edge [e] (789)
    }
    (1) edge [ev, bend right=90] (c1)
    (1) edge [ev, bend left=90] (c1)
    \foreach \i/\j in {2/3,3/4,4/2,7/8,8/9,9/7}{
    (\i) edge [ev] (\j)
    }
    \foreach \i/\j in {1/2,3/7,4/8}{
    (\i) edge [es] (\j)
    };
\end{tikzpicture}
}

% ------------ 2-coloured graphs --------------

\newcommand{\rtedge}{
\begin{tikzpicture}[x=2ex,y=2ex,baseline={([yshift=-.59ex]current bounding box.center)}] 
\node [v]	(v)	at (0,0) 	{};
\node [vb]	(1)	at (-1,0)	{};
\node [vb]	(2)	at (1,0)	{};
\path
\foreach \i in {1,2}{
    (\i) edge [e] (v)
    }
(1)	edge [ev,bend left=35]	(2)
(1)	edge [ev,bend right=35]	(2);
\end{tikzpicture}
}

\newcommand{\edgevgb}{
\begin{tikzpicture}[x=2ex,y=2ex,baseline={([yshift=-.59ex]current bounding box.center)}]
\node [vb]	(1)	at (0,1)	{};
\node [vb]	(2)	at (0,-1)	{};
\path
(1)	edge [ev,bend left=30]	(2)
(1)	edge [ev,bend right=30]	(2);
\end{tikzpicture}
}

\newcommand{\edgevg}{
\begin{tikzpicture}[x=2ex,y=2ex,baseline={([yshift=-.59ex]current bounding box.center)}]
\node [vb]	(1)	at (1,0)	{};
\node [vb]	(2)	at (-1,0)	{};
\path
(1)	edge [ev,bend left=30]	(2)
(1)	edge [ev,bend right=30]	(2);
\end{tikzpicture}
}

\newcommand{\edgevgr}{
\begin{tikzpicture}[x=2ex,y=2ex,baseline={([yshift=-.59ex]current bounding box.center)}]
\node [vb]	(1)	at (1,0)	{};
\node [vb]	(2)	at (-1,0)	{};
\node at (0,0) {...};
\path
(1)	edge [ev,bend left=50] 	(2)
(1)	edge [ev,bend left=30] 	(2)
(1)	edge [ev,bend right=30] (2)
(1)	edge [ev,bend right=50]	(2);
\end{tikzpicture}
}

\newcommand{\mapthreevertex}{
\begin{tikzpicture}[x=2ex,y=2ex,baseline={([yshift=-.59ex]current bounding box.center)}] 
\node [v]	(v) at (0,0) 	{};
\node [vb]	(1)	at (-1,0)	{};
\node [vb]	(2)	at (.6,-1)	{};
\node [vb]	(3)	at (.6,1)	{};
\path
\foreach \i in {1,2,3}{
    (\i) edge [e] (v)
    }
\foreach \i/\j in {1/2,2/3,3/1}{
    (\i) edge [ev] (\j)
    };
\end{tikzpicture}
}

\newcommand{\onevg}{
\begin{tikzpicture}[x=1.2ex,y=1.2ex,baseline={([yshift=-.59ex]current bounding box.center)}] 
    \node [c]	(c1)	at (-3,0) 	{};
    \node [vb]	(1)	at (-2,0)	{};    
    \path
    (1) edge [ev, bend right=90] (c1)
    (1) edge [ev, bend left=90] (c1);
\end{tikzpicture}
}

\newcommand{\threevg}{
\begin{tikzpicture}[x=.7ex,y=.7ex,baseline={([yshift=-.59ex]current bounding box.center)}] 
\node [vb]	(1)	at (-1,0)	{};
\node [vb]	(2)	at (.6,-1)	{};
\node [vb]	(3)	at (.6,1)	{};
\path
\foreach \i/\j in {1/2,2/3,3/1}{
    (\i) edge [ev] (\j)
    };
\end{tikzpicture}
}

\newcommand{\rtvf}{
\begin{tikzpicture}[x=2ex,y=2ex,baseline={([yshift=-.59ex]current bounding box.center)}]
\scriptsize{
\node [v]	(v)	at (0,0) 	{};
\node [vb]	(1)	at (-1,1)	{};
\node [vb]	(2)	at (-1,-1)	{};
\node [vb]	(3)	at (1,-1)	{};
\node [vb]	(4)	at (1,1)	{};
\path
\foreach \i in {1,2,3,4}{
    (\i) edge [e] (v)
    }
(1) edge [ev]  node [c, label=left:$c$] {} (2)
\foreach \i/\j in {2/3,3/4,4/1}{
    (\i) edge [ev] (\j)
    };
}
\end{tikzpicture}
}

\newcommand{\rtvfg}{
\begin{tikzpicture}[x=.7ex,y=.7ex,baseline={([yshift=-.59ex]current bounding box.center)}]
\node [vb]	(1)	at (-1,1)	{};
\node [vb]	(2)	at (-1,-1)	{};
\node [vb]	(3)	at (1,-1)	{};
\node [vb]	(4)	at (1,1)	{};
\path
\foreach \i/\j in {1/2,2/3,3/4,4/1}{
    (\i) edge [ev] (\j)
    };
\end{tikzpicture}
}

\newcommand{\rttadpole}{
\begin{tikzpicture}[x=2ex,y=2ex,baseline={([yshift=-1.2ex]current bounding box.center)}]
\node [v]	(v)	at (0,0) 	{};
\node [vb]	(1)	at (-1,1)	{};
\node [vb]	(2)	at (-1,-1)	{};
\node [vb]	(3)	at (1,-1)	{};
\node [vb]	(4)	at (1,1)	{};
\path
\foreach \i in {1,2,3,4}{
    (\i) edge [e] (v)
    }
\foreach \i/\j in {1/2,2/3,3/4,4/1}{
    (\i) edge [ev] (\j)
    }
(1)	edge [es,bend left=60]	(4);
\end{tikzpicture}
}

\newcommand{\rttadpolec}{
\begin{tikzpicture}[x=2ex,y=2ex,baseline={([yshift=-1.2ex]current bounding box.center)}]
\scriptsize{
\node [v]	(v)	at (0,0) 	{};
\node [vb]	(1)	at (-1,1)	{};
\node [vb]	(2)	at (-1,-1)	{};
\node [vb]	(3)	at (1,-1)	{};
\node [vb]	(4)	at (1,1)	{};
\path
\foreach \i in {1,2,3,4}{
    (\i) edge [e] (v)
    }
(1) edge [ev]  node [c, label=left:$c$] {} (2)
\foreach \i/\j in {2/3,3/4,4/1}{
    (\i) edge [ev] (\j)
    }
(1)	edge [es,bend left=60]	(4);
}
\end{tikzpicture}
}

\newcommand{\rttadpolepq}{
\begin{tikzpicture}[x=2ex,y=2ex,baseline={([yshift=-1.2ex]current bounding box.center)}]
\scriptsize{
\node [v]	(v)	at (0,0) 	{};
\node [vb]	(1)	at (-1,1)	{};
\node [vb]	(2)	at (-1,-1)	{};
\node [vb]	(3)	at (1,-1)	{};
\node [vb]	(4)	at (1,1)	{};
\path
\foreach \i in {1,2,3,4}{
    (\i) edge [e] (v)
    }
(1) edge [ev]  node [c, label=left:$p_1$] {} (2)
(1) edge [ev]  node [c, label=above:$q_2$]{} (4)
\foreach \i/\j in {2/3,3/4,4/1}{
    (\i) edge [ev] (\j)
    };
%(1)	edge [es,bend left=60]	(4);
\draw [es] (1) arc [start angle=180, end angle=0, radius=1];
}
\end{tikzpicture}
}

\newcommand{\rttadpoleb}{
\begin{tikzpicture}[x=2ex,y=2ex,baseline={([yshift=-.59ex]current bounding box.center)}]
\scriptsize{
\node [v]	(v)	at (0,0) 	{};
\node [vb]	(1)	at (-1,1)	{};
\node [vb]	(2)	at (-1,-1)	{};
\node [vb]	(3)	at (1,-1)	{};
\node [vb]	(4)	at (1,1)	{};
\path
\foreach \i in {1,2,3,4}{
    (\i) edge [e] (v)
    }
(1) edge [ev]  node [c, label=above:$c$] {} (4)
\foreach \i/\j in {1/2,2/3,3/4}{
    (\i) edge [ev] (\j)
    }
(2)	edge [es,bend right=60]	(3);
}
\end{tikzpicture}
}

\newcommand{\rttadpolebpq}{
\begin{tikzpicture}[x=2ex,y=2ex,baseline={([yshift=.49ex]current bounding box.center)}]
\scriptsize{
\node [v]	(v)	at (0,0) 	{};
\node [vb]	(1)	at (-1,1)	{};
\node [vb]	(2)	at (-1,-1)	{};
\node [vb]	(3)	at (1,-1)	{};
\node [vb]	(4)	at (1,1)	{};
\path
\foreach \i in {1,2,3,4}{
    (\i) edge [e] (v)
    }
(1) edge [ev]  node [c, label=left:$p_2$] {} (2)
(2) edge [ev]  node [c, label=below:$q_1$] {} (3)
\foreach \i/\j in {3/4,4/1}{
    (\i) edge [ev] (\j)
    };
%(2)	edge [es,bend right=60]	(3);
\draw [es] (2) arc [start angle=180, end angle=360, radius=1];
}
\end{tikzpicture}
}

\newcommand{\rtsunrisec}{
\begin{tikzpicture}[x=2ex,y=2ex,baseline={([yshift=-.6ex]current bounding box.center)}]
\scriptsize{
\begin{scope}[rotate=-45]
\node [v]	(v1)at (0,0) 	{};
\node [vb]	(1)	at (-1,1)	{};
\node [vb]	(2)	at (-1,-1)	{};
\node [vb]	(3)	at (1,-1)	{};
\node [vb]	(4)	at (1,1)	{};
\end{scope}
\begin{scope}[xshift=1.5cm,rotate=-45]
\node [v]	(v2)at (0,0) 	{};
\node [vb]	(5)	at (-1,1)	{};
\node [vb]	(6)	at (-1,-1)	{};
\node [vb]	(7)	at (1,-1)	{};
\node [vb]	(8)	at (1,1)	{};
\end{scope}
\path
\foreach \i in {1,2,3,4}{
    (\i) edge [e] (v1)
    }
\foreach \i in {5,6,7,8}{
    (\i) edge [e] (v2)
    }
(1) edge [ev]  node [c, label=135:$c$] {} (2)
(8) edge [ev]  node [c, label=45:$c$] {} (5)
\foreach \i/\j in {2/3,3/4,4/1,5/6,6/7,7/8}{
    (\i) edge [ev] (\j)
    }
\foreach \i/\j in {1/5,3/7,4/6}{
    (\i) edge [es] (\j)
    };
}
\end{tikzpicture}
}

\newcommand{\rtsunrisepq}{
\begin{tikzpicture}[x=2ex,y=2ex,baseline={([yshift=-.6ex]current bounding box.center)}]
\scriptsize{
\begin{scope}[rotate=-45]
\node [v]	(v1)at (0,0) 	{};
\node [vb]	(1)	at (-1,1)	{};
\node [vb]	(2)	at (-1,-1)	{};
\node [vb]	(3)	at (1,-1)	{};
\node [vb]	(4)	at (1,1)	{};
\end{scope}
\begin{scope}[xshift=1.5cm,rotate=-45]
\node [v]	(v2)at (0,0) 	{};
\node [vb]	(5)	at (-1,1)	{};
\node [vb]	(6)	at (-1,-1)	{};
\node [vb]	(7)	at (1,-1)	{};
\node [vb]	(8)	at (1,1)	{};
\end{scope}
\path
\foreach \i in {1,2,3,4}{
    (\i) edge [e] (v1)
    }
\foreach \i in {5,6,7,8}{
    (\i) edge [e] (v2)
    }
(1) edge [ev]  node [c, label=135:$p_1$] {} (2)
(2) edge [ev]  node [c, label=225:$p_2$] {} (3)
(3) edge [ev]  node [c, label=right:$q_1$] {} (4)
(4) edge [ev]  node [c, label=right:$q_2$] {} (1)
\foreach \i/\j in {5/6,6/7,7/8,8/5}{
    (\i) edge [ev] (\j)
    }
\foreach \i/\j in {1/5,3/7,4/6}{
    (\i) edge [es] (\j)
    };
}
\end{tikzpicture}
}

\newcommand{\rtsunrisesub}[1]{
\begin{tikzpicture}[x=2ex,y=2ex,baseline={([yshift=-.6ex]current bounding box.center)}]
\scriptsize{
\begin{scope}[rotate=-45]
\node [v]	(v1)at (0,0) 	{};
\node [vb]	(1)	at (-1,1)	{};
\node [vb]	(2)	at (-1,-1)	{};
\node [vb]	(3)	at (1,-1)	{};
\node [vb]	(4)	at (1,1)	{};
\end{scope}
\begin{scope}[xshift=1.5cm,rotate=-45]
\node [v]	(v2)at (0,0) 	{};
\node [vb]	(5)	at (-1,1)	{};
\node [vb]	(6)	at (-1,-1)	{};
\node [vb]	(7)	at (1,-1)	{};
\node [vb]	(8)	at (1,1)	{};
\end{scope}
\path
\foreach \i in {1,2,3,4}{
    (\i) edge [e] (v1)
    }
\foreach \i in {5,6,7,8}{
    (\i) edge [e] (v2)
    }
(1) edge [ev]  node [c, label=135:$c$] {} (2)
(8) edge [ev]  node [c, label=45:$c$] {} (5)
\foreach \i/\j in {2/3,3/4,4/1,5/6,6/7,7/8}{
    (\i) edge [ev] (\j)
    }
\foreach \i/\j in {#1}{
    (\i) edge [es] (\j)
    };
}
\end{tikzpicture}
}

\newcommand{\rtfisha}{
\begin{tikzpicture}[x=2ex,y=2ex,baseline={([yshift=-1.2ex]current bounding box.center)}]
\scriptsize{
\begin{scope}[rotate=-90]
\node [v]	(v1)at (0,0) 	{};
\node [vb]	(1)	at (-1,1)	{};
\node [vb]	(2)	at (-1,-1)	{};
\node [vb]	(3)	at (1,-1)	{};
\node [vb]	(4)	at (1,1)	{};
\end{scope}
\begin{scope}[xshift=1.3cm]
\node [v]	(v2)at (0,0) 	{};
\node [vb]	(5)	at (-1,1)	{};
\node [vb]	(6)	at (-1,-1)	{};
\node [vb]	(7)	at (1,-1)	{};
\node [vb]	(8)	at (1,1)	{};
\end{scope}
\path
\foreach \i in {1,2,3,4}{
    (\i) edge [e] (v1)
    }
\foreach \i in {5,6,7,8}{
    (\i) edge [e] (v2)
    }
(1) edge [ev]  node [c, label=above:$c$] {} (2)
(8) edge [ev]  node [c, label=above:$c$] {} (5)
\foreach \i/\j in {2/3,3/4,4/1,5/6,6/7,7/8}{
    (\i) edge [ev] (\j)
    }
\foreach \i/\j in {1/5,4/6}{
    (\i) edge [es] (\j)
    };
}
\end{tikzpicture}
}

\newcommand{\rtfishpq}[3]{
\begin{tikzpicture}[x=2ex,y=2ex,baseline={([yshift=-.59ex]current bounding box.center)}]
\scriptsize{
\begin{scope}[rotate=-90]
\node [v]	(v1)at (0,0) 	{};
\node [vb]	(1)	at (-1,1)	{};
\node [vb]	(2)	at (-1,-1)	{};
\node [vb]	(3)	at (1,-1)	{};
\node [vb]	(4)	at (1,1)	{};
\end{scope}
\begin{scope}[xshift=1.3cm]
\node [v]	(v2)at (0,0) 	{};
\node [vb]	(5)	at (-1,1)	{};
\node [vb]	(6)	at (-1,-1)	{};
\node [vb]	(7)	at (1,-1)	{};
\node [vb]	(8)	at (1,1)	{};
\end{scope}
\path
\foreach \i in {1,2,3,4}{
    (\i) edge [e] (v1)
    }
\foreach \i in {5,6,7,8}{
    (\i) edge [e] (v2)
    }
(1) edge [ev]  node [c, label=above:$#1$] {} (2)
(3) edge [ev]  node [c, label=below:$#3$] {} (4)
(1) edge [ev]  node [c, label=right:$#2$] {} (4)
\foreach \i/\j in {2/3,3/4,4/1,5/6,6/7,7/8,8/5}{
    (\i) edge [ev] (\j)
    }
\foreach \i/\j in {1/5,4/6}{
    (\i) edge [es] (\j)
    };
}
\end{tikzpicture}
}

\newcommand{\rtfishb}{
\begin{tikzpicture}[x=2ex,y=2ex,baseline={([yshift=-.59ex]current bounding box.center)}]
\scriptsize{
\node [v]	(v1)at (0,0) 	{};
\node [vb]	(1)	at (-1,1)	{};
\node [vb]	(2)	at (-1,-1)	{};
\node [vb]	(3)	at (1,-1)	{};
\node [vb]	(4)	at (1,1)	{};
\begin{scope}[xshift=1.3cm]
\node [v]	(v2)at (0,0) 	{};
\node [vb]	(5)	at (-1,1)	{};
\node [vb]	(6)	at (-1,-1)	{};
\node [vb]	(7)	at (1,-1)	{};
\node [vb]	(8)	at (1,1)	{};
\end{scope}
\path
\foreach \i in {1,2,3,4}{
    (\i) edge [e] (v1)
    }
\foreach \i in {5,6,7,8}{
    (\i) edge [e] (v2)
    }
(1) edge [ev]  node [c, label=left:$c$] {} (2)
(5) edge [ev]  node [c, label=left:$c$] {} (6)
\foreach \i/\j in {2/3,3/4,4/1,6/7,7/8,8/5}{
    (\i) edge [ev] (\j)
    }
\foreach \i/\j in {4/5,3/6}{
    (\i) edge [es] (\j)
    };
}
\end{tikzpicture}
}

\newcommand{\mapa}{
\begin{tikzpicture}[x=2ex,y=2ex,baseline={([yshift=-.59ex]current bounding box.center)}] 
\node [v]	(v)	at (0,0) 	{};
\node [vb]	(1)	at (-1,1)	{};
\node [vb]	(2)	at (-1,-1)	{};
\node [vb]	(3)	at (1,-1)	{};
\node [vb]	(4)	at (1,1)	{};
\path
\foreach \i in {1,2,3,4}{
    (\i) edge [e] (v)
    }
\foreach \i/\j in {1/2,3/4}{
   (\i)	edge [ev,bend left=30]	(\j)
   (\i)	edge [ev,bend right=30]	(\j)
   };
\end{tikzpicture}
}

\newcommand{\mapb}{
\begin{tikzpicture}[x=2ex,y=2ex,baseline={([yshift=-.59ex]current bounding box.center)}] 
\node [v]	(v1)at (0,0) 	{};
\node [v]	(v2)at (2.6,0) 	{};
\node [vb]	(1)	at (-1,0)	{};
\node [vb]	(2)	at (.6,-1)	{};
\node [vb]	(3)	at (.6,1)	{};
\node [vb]	(9)	at (3.6,0)	{};
\node [vb]	(8)	at (2,1)	{};
\node [vb]	(7)	at (2,-1)	{};
\path
\foreach \i in {1,2,3}{
    (\i) edge [e] (v1)
    }
\foreach \i in {7,8,9}{
    (\i) edge [e] (v2)
    }
\foreach \i/\j in {1/2,2/3,3/1,7/8,8/9,9/7}{
    (\i) edge [ev] (\j)
    }
\foreach \i/\j in {2/7,3/8}{
    (\i) edge [es] (\j)
    };
\end{tikzpicture}
}

\newcommand{\mapc}{
\begin{tikzpicture}[x=2ex,y=2ex,baseline={([yshift=-.59ex]current bounding box.center)}]
\node [v]	(v1)	at (0,0) 	{};
\node [vb]	(1)	at (-1,1)	{};
\node [vb]	(2)	at (-1,-1)	{};
\node [vb]	(3)	at (1,-1)	{};
\node [vb]	(4)	at (1,1)	{};
\begin{scope}[xshift=7ex]
\node [v]	(v2)	at (0,0) 	{};
\node [vb]	(5)	at (-1,1)	{};
\node [vb]	(6)	at (-1,-1)	{};
\node [vb]	(7)	at (1,-1)	{};
\node [vb]	(8)	at (1,1)	{};
\end{scope}
\path
\foreach \i in {1,2,3,4}{
    (\i) edge [e] (v1)
    }
\foreach \i in {5,6,7,8}{
    (\i) edge [e] (v2)
    }
\foreach \i/\j in {1/2,2/3,3/4,4/1,5/6,6/7,7/8,8/5}{
    (\i) edge [ev] (\j)
    }
\foreach \i/\j in {4/8,7/3}{
    (\i) edge [es, bend left=30] (\j)
    };
\end{tikzpicture}
}

\newcommand{\mapd}{
\begin{tikzpicture}[x=2ex,y=2ex,baseline={([yshift=-.59ex]current bounding box.center)}]
\node [v]	(v1)at (0,0) 	{};
\node [v]	(v2)at (2.4,0) 	{};
\node [vb]	(1)	at (-1,0)	{};
\node [vb]	(2)	at (.6,-1)	{};
\node [vb]	(3)	at (.6,1)	{};
\node [vb]	(4)	at (1.4,0)	{};
\node [vb]	(5)	at (3,-1)	{};
\node [vb]	(6)	at (3,1)	{};
\path
\foreach \i in {1,2,3}{
    (\i) edge [e] (v1)
    }
\foreach \i in {4,5,6}{
    (\i) edge [e] (v2)
    }
\foreach \i/\j in {1/2,2/3,3/1,4/5,5/6,6/4}{
    (\i) edge [ev] (\j)
    }
\foreach \i/\j in {2/5,3/6}{
    (\i) edge [es] (\j)
    };
\end{tikzpicture}
}

\newcommand{\maptorus}{
\begin{tikzpicture}[x=2ex,y=2ex,baseline={([yshift=-.59ex]current bounding box.center)}]
\node [v]	(v3)	at (0,0) 	{};
\node [v]	(v4)	at (2,0) 	{};
\node [vb]	(11)	at (-1,0)	{};
\node [vb]	(12)	at (.6,-1)	{};
\node [vb]	(13)	at (.6,1)	{};
\node [vb]	(9)	at (3,0)	{};
\node [vb]	(8)	at (1.4,1)	{};
\node [vb]	(7)	at (1.4,-1)	{};
\begin{scope}[yshift=5ex]
\node [v]	(v1)	at (0,0) 	{};
\node [v]	(v2)	at (2.4,0) 	{};
\node [vb]	(1)	at (-1,0)	{};
\node [vb]	(2)	at (.6,-1)	{};
\node [vb]	(3)	at (.6,1)	{};
\node [vb]	(4)	at (1.4,0)	{};
\node [vb]	(5)	at (3,-1)	{};
\node [vb]	(6)	at (3,1)	{};
\end{scope}
\path
\foreach \i/\j in {1/v1,2/v1,3/v1,4/v2,5/v2,6/v2,11/v3,12/v3,13/v3,7/v4,8/v4,9/v4}{
    (\i) edge [e] (\j)
    }
\foreach \i/\j in {1/2,2/3,3/1,4/5,5/6,6/4,7/8,8/9,9/7,11/12,12/13,13/11}{
    (\i) edge [ev] (\j)
    }
\foreach \i/\j in {2/5,3/6,1/11,12/7,13/8}{
    (\i) edge [es] (\j)
    }
(4) edge [es,sloped] (9);
\end{tikzpicture}
}

\newcommand{\mapcon}{
\begin{tikzpicture}[x=2ex,y=2ex,baseline={([yshift=-.59ex]current bounding box.center)}]
\draw [ev] (0,1.8) circle (.5ex); 
\draw [ev] (2,1.8) circle (.5ex); 
\node [v]	(v3)at (0,0) 	{};
\node [v]	(v4)at (2,0) 	{};
\node [vb]	(1)	at (-1,0)	{};
\node [vb]	(2)	at (.6,-1)	{};
\node [vb]	(3)	at (.6,1)	{};
\node [vb]	(9)	at (3,0)	{};
\node [vb]	(8)	at (1.4,1)	{};
\node [vb]	(7)	at (1.4,-1)	{};
\node [v]	(v2)at (1,1.5) 	{};
\node [vb]	(4)	at (0,1.5)	{};
\node [vb]	(5)	at (2,1.5)	{};
\path
\foreach \i/\j in {4/v2,5/v2,1/v3,2/v3,3/v3,7/v4,8/v4,9/v4}{
    (\i) edge [e] (\j)
    }
\foreach \i/\j in {1/2,2/3,3/1,7/8,8/9,9/7}{
    (\i) edge [ev] (\j)
    }
\foreach \i/\j in {2/7,3/8,1/4,9/5}{
    (\i) edge [es] (\j)
    };
\end{tikzpicture}
}

%--------------- r=3 coloured graphs ------------------

\newcommand{\rhvfc}{
\begin{tikzpicture}[rotate=90, x=2ex,y=2ex,baseline={([yshift=-.59ex]current bounding box.center)}] 
\scriptsize{
\node [v]	(1)	at (0,0)	{};
\node [vb]	(b1)	at (-1,1)	{};
\node [vb]	(w1)	at (-1,-1)	{};
\node [vb]	(b2)	at (1,-1)	{};
\node [vb]	(w2)	at (1,1)	{};
\path
\foreach \i/\j in {1/2}{
   	(w\i) edge [ev]   (b\j)
	(b\i) edge [ev]  node [c, label=left:$c$] {} (w\j)
	}
\foreach \i in {1,2}{
	(w\i)	edge [ev,bend left=30]	(b\i)
	(w\i)	edge [ev,bend right=30]	(b\i)
	}
\foreach \i in {w1,b1,w2,b2}{
   	(\i) edge [e] (1)
	};
}
\end{tikzpicture}
}

\newcommand{\rhvfg}{
\begin{tikzpicture}[rotate=-90,x=.7ex,y=.7ex,baseline={([yshift=-.59ex]current bounding box.center)}] 
\scriptsize{
\node [vb]	(b1)	at (-1,1)	{};
\node [vb]	(w1)	at (-1,-1)	{};
\node [vb]	(b2)	at (1,-1)	{};
\node [vb]	(w2)	at (1,1)	{};
\path
\foreach \i/\j in {1/2}{
   	(w\i) edge [ev]   (b\j)
	(b\i) edge [ev]  node [c, label=right:$c$] {} (w\j)
	}
\foreach \i in {1,2}{
	(w\i)	edge [ev,bend left=30]	(b\i)
	(w\i)	edge [ev,bend right=30]	(b\i)
	};
}
\end{tikzpicture}
}

\newcommand{\rhtadpolea}{
\begin{tikzpicture}[rotate=90, x=2ex,y=2ex,baseline={([yshift=-1.2ex]current bounding box.center)}] 
\scriptsize{
\node [v]	(1)	    at (0,0)	{};
\node [vb]	(b1)	at (-1,1)	{};
\node [vb]	(w1)	at (-1,-1)	{};
\node [vb]	(b2)	at (1,-1)	{};
\node [vb]	(w2)	at (1,1)	{};
\path
\foreach \i/\j in {1/2}{
   	(w\i) edge [ev]   (b\j)
	(b\i) edge [ev]  node [c, label=left:$c$] {} (w\j)
	}
\foreach \i in {1,2}{
	(w\i)	edge [ev,bend left=30]	(b\i)
	(w\i)	edge [ev,bend right=30]	(b\i)
	}
\foreach \i in {w1,b1,w2,b2}{
   	(\i) edge [e] (1)
	}
(w2)	edge [es,bend left=90]	(b2);
}
\end{tikzpicture}
}

\newcommand{\rhtadpoleapq}{
\begin{tikzpicture}[rotate=90, x=2ex,y=2ex,baseline={([yshift=-1.2ex]current bounding box.center)}] 
\scriptsize{
\node [v]	(1)	    at (0,0)	{};
\node [vb]	(b1)	at (-1,1)	{};
\node [vb]	(w1)	at (-1,-1)	{};
\node [vb]	(b2)	at (1,-1)	{};
\node [vb]	(w2)	at (1,1)	{};
\path
\foreach \i/\j in {1/2}{
   	(w\i) edge [ev]   (b\j)
	(b\i) edge [ev]  node [c, label=left:$p_1$] {} (w\j)
	}
\foreach \i in {1,2}{
	(w\i)	edge [ev,bend left=30]	(b\i)
	(w\i)	edge [ev,bend right=30]	(b\i)
	}
\foreach \i in {w1,b1,w2,b2}{
   	(\i) edge [e] (1)
	}
(w2)	edge [es,bend left=90]	(b2);
}
\end{tikzpicture}
}


\newcommand{\rhtadpoleb}{
\begin{tikzpicture}[x=2ex,y=2ex,baseline={([yshift=-.3ex]current bounding box.center)}] 
\scriptsize{
\node [v]	(1)	    at (0,0)	{};
\node [vb]	(b1)	at (-1,1)	{};
\node [vb]	(w1)	at (-1,-1)	{};
\node [vb]	(b2)	at (1,-1)	{};
\node [vb]	(w2)	at (1,1)	{};
\path
\foreach \i/\j in {1/2}{
   	(w\i) edge [ev]  node [c, label=below:$c$] {} (b\j)
	(b\i) edge [ev]   (w\j)
	}
\foreach \i in {1,2}{
	(w\i)	edge [ev,bend left=30]	(b\i)
	(w\i)	edge [ev,bend right=30]	(b\i)
	}
\foreach \i in {w1,b1,w2,b2}{
   	(\i) edge [e] (1)
	}
(b1)	edge [es,bend left=60]	(w2);
}
\end{tikzpicture}
}

\newcommand{\rhtadpolebpq}{
\begin{tikzpicture}[x=2ex,y=2ex,baseline={([yshift=-.3ex]current bounding box.center)}] 
\scriptsize{
\node [v]	(1)	    at (0,0)	{};
\node [vb]	(b1)	at (-1,1)	{};
\node [vb]	(w1)	at (-1,-1)	{};
\node [vb]	(b2)	at (1,-1)	{};
\node [vb]	(w2)	at (1,1)	{};
\path
\foreach \i/\j in {1/2}{
   	(w\i) edge [ev]  (b\j)
	(b\i) edge [ev]  node [c, label=above:$q_1$] {} (w\j)
	}
(w1)	edge [ev,bend left=30] node [c, label=left:{$p_2,p_3$}] {}	(b1)
(w1)	edge [ev,bend right=30]	(b1)
\foreach \i in {2}{
	(w\i)	edge [ev,bend left=30]	(b\i)
	(w\i)	edge [ev,bend right=30]	(b\i)
	}
\foreach \i in {w1,b1,w2,b2}{
   	(\i) edge [e] (1)
	};
%(b1)	edge [es,bend left=60]	(w2);
\draw [es] (b1) arc [start angle=180, end angle=0, radius=1];
}
\end{tikzpicture}
}

\newcommand{\rhsunrise}[5]{
\begin{tikzpicture}[x=2ex,y=2ex,baseline={([yshift=-.6ex]current bounding box.center)}]
\scriptsize{
\begin{scope}[rotate=-45]
\node [v]	(v1)at (0,0) 	{};
\node [vb]	(1)	at (-1,1)	{};
\node [vb]	(2)	at (-1,-1)	{};
\node [vb]	(3)	at (1,-1)	{};
\node [vb]	(4)	at (1,1)	{};
\end{scope}
\begin{scope}[xshift=1.5cm,rotate=-45]
\node [v]	(v2)at (0,0) 	{};
\node [vb]	(5)	at (-1,1)	{};
\node [vb]	(6)	at (-1,-1)	{};
\node [vb]	(7)	at (1,-1)	{};
\node [vb]	(8)	at (1,1)	{};
\end{scope}
\path
\foreach \i in {1,2,3,4}{
    (\i) edge [e] (v1)
    }
\foreach \i in {5,6,7,8}{
    (\i) edge [e] (v2)
    }
(1) edge [ev]  node [c, label=135:$#1$] {} (2)
(2) edge [ev, bend left=30]  node [c, label=225:$#2$] {} (3)
(2) edge [ev, bend right=30] (3)
(4) edge [ev, bend right=30]  node [c, label=right:$#3$] {} (1)
(4) edge [ev, bend left=30]   (1)
(3) edge [ev]  node [c, label=right:$#4$] {} (4)
(5) edge [ev]  node [c, label=45:$#5$] {} (8)
\foreach \i/\j in {6/7,8/5}{
    (\i) edge [ev] (\j)
    }
\foreach \i\j in {5/6,7/8}{
	(\i)	edge [ev,bend left=30]	(\j)
	(\i)	edge [ev,bend right=30]	(\j)
	}
\foreach \i/\j in {1/5,3/7,4/6}{
    (\i) edge [es] (\j)
    };
}
\end{tikzpicture}
}

\newcommand{\rhfish}[4]{
\begin{tikzpicture}[x=2ex,y=2ex,baseline={([yshift=-.59ex]current bounding box.center)}]
\scriptsize{
\begin{scope}[rotate=-90]
\node [v]	(v1)at (0,0) 	{};
\node [vb]	(1)	at (-1,1)	{};
\node [vb]	(2)	at (-1,-1)	{};
\node [vb]	(3)	at (1,-1)	{};
\node [vb]	(4)	at (1,1)	{};
\end{scope}
\begin{scope}[xshift=1.8cm]
\node [v]	(v2)at (0,0) 	{};
\node [vb]	(5)	at (-1,1)	{};
\node [vb]	(6)	at (-1,-1)	{};
\node [vb]	(7)	at (1,-1)	{};
\node [vb]	(8)	at (1,1)	{};
\end{scope}
\path
\foreach \i in {1,2,3,4}{
    (\i) edge [e] (v1)
    }
\foreach \i in {5,6,7,8}{
    (\i) edge [e] (v2)
    }
(1) edge [ev]  node [c, label=above:$#1$] {} (2)
(1) edge [ev,bend left=30]  node [c, label=right:$#2$] {} (4)
(1) edge [ev,bend right=30] (4)
(3) edge [ev]  node [c, label=below:$#3$] {} (4)
(5) edge [ev]  node [c, label=above:$#4$] {} (8)
\foreach \i/\j in {3/4,6/7,8/5}{
    (\i) edge [ev] (\j)
    }
\foreach \i\j in {2/3,5/6,7/8}{
	(\i)	edge [ev,bend left=30]	(\j)
	(\i)	edge [ev,bend right=30]	(\j)
	}
\foreach \i/\j in {1/5,4/6}{
    (\i) edge [es] (\j)
    };
}
\end{tikzpicture}
}

%--------------- r=4 coloured graphs ------------------

\newcommand{\cvtvg}{
\begin{tikzpicture}[x=1ex,y=1ex,baseline={([yshift=-.59ex]current bounding box.center)}] 
\node [vb]	(1)	at (0,1)	{};
\node [vb]	(2)	at (0,-1)	{};
\path
\foreach \i/\j in {1/2,2/1}{
   (\i)	edge [ev,bend left=15]	(\j)
   (\i)	edge [ev,bend left=40]	(\j)
   };
\end{tikzpicture}
}

\newcommand{\cvt}{
\begin{tikzpicture}[x=2ex,y=2ex,baseline={([yshift=-.59ex]current bounding box.center)}] 
\node [v]	(v)	at (0,0)	{};
\node [vb]	(1)	at (1,0)	{};
\node [vb]	(2)	at (-1,0)	{};
\path
\foreach \i in {1,2}{
    (\i) edge [e] (v)
    }
\foreach \i/\j in {1/2,2/1}{
   (\i)	edge [ev,bend left=30]	(\j)
   (\i)	edge [ev,bend left=50]	(\j)
   };
\end{tikzpicture}
}

\newcommand{\cvfvg}{
\begin{tikzpicture}[x=1ex,y=1ex,baseline={([yshift=-.59ex]current bounding box.center)}] 
\scriptsize{
%\node [v]	(1)	at (0,0)	{};
\node [vb, label=above:]	(b1)	at (-1,1)	{};
\node [vb, label=below:]	(w1)	at (-1,-1)	{};
\node [vb, label=below:]	(b2)	at (1,-1)	{};
\node [vb, label=above:]	(w2)	at (1,1)	{};
\path
\foreach \i/\j in {1/2}{
   	(w\i) edge [ev]  node [c, label=below:$\ell$] {} (b\j)
	(b\i) edge [ev]   (w\j)
	}
\foreach \i in {1,2}{
	(w\i)   edge [ev]				(b\i)
	(w\i)	edge [ev,bend left=30]	(b\i)
	(w\i)	edge [ev,bend right=30]	(b\i)
	};
% \foreach \i in {w1,b1,w2,b2}{
%   	(\i) edge [e] (1)
% 	};
}
\end{tikzpicture}
}

\newcommand{\cvfnvg}{
\begin{tikzpicture}[x=1ex,y=1ex,baseline={([yshift=-.59ex]current bounding box.center)}] 
\scriptsize{
%\node [v]	(1)	at (0,0)	{};
\node [vb, label=above:]	(b1)	at (-1,1)	{};
\node [vb, label=below:]	(w1)	at (-1,-1)	{};
\node [vb, label=below:]	(b2)	at (1,-1)	{};
\node [vb, label=above:]	(w2)	at (1,1)	{};
\path
\foreach \i/\j in {1/2,2/1}{
   	%(w\i) edge [ev]   (b\j)
   	%(w\i)	edge [ev,bend left=30]	(b\i)
   	(w\i) edge [ev,bend left=30]  (b\j)
   	(w\i) edge [ev,bend right=30] (b\j)
	%(b\i) edge [ev]  node [c, label=above:$\ell$] {} (w\j)
	}
\foreach \i in {1,2}{
	%(w\i)   edge 	[ev]				(b\i)
	(w\i)	edge [ev,bend left=30]  (b\i)
	(w\i)	edge [ev,bend right=30]	(b\i)
	}

\foreach \i in {w1,b1,w2,b2}{
  	%(\i) edge [e] (1)
	};
}
\end{tikzpicture}
}

\newcommand{\cvf}{
\begin{tikzpicture}[scale=2,x=2ex,y=2ex,baseline={([yshift=-.59ex]current bounding box.center)}] 
\scriptsize{
\node [v]	(1)	at (0,0)	{};
\node [vb, label=above:]	(b1)	at (-1,1)	{};
\node [vb, label=below:]	(w1)	at (-1,-1)	{};
\node [vb, label=below:]	(b2)	at (1,-1)	{};
\node [vb, label=above:]	(w2)	at (1,1)	{};
\path
\foreach \i/\j in {1/2}{
   	(w\i) edge [ev]   (b\j)
	%(b\i) edge [ev]  node [c, label=above:$\ell$] {} (w\j)
	(b\i) edge [ev]  node [c] {} (w\j)
	}
\foreach \i in {1,2}{
	(w\i)   edge 	[ev]				(b\i)
	(w\i)	edge [ev,bend left=30]	(b\i)
	(w\i)	edge [ev,bend right=30]	(b\i)
	}
\foreach \i in {w1,b1,w2,b2}{
   	(\i) edge [e] (1)
	};
}
\end{tikzpicture}
}

\newcommand{\cvfneu}{
\begin{tikzpicture}[scale=2,x=2ex,y=2ex,baseline={([yshift=-.59ex]current bounding box.center)}] 
\scriptsize{
%\node [v]	(1)	at (0,0)	{};
\node [wv, label=above:]	(b1)	at (-1,1)	{};
\node [bv, label=below:]	(w1)	at (-1,-1)	{};
\node [wv, label=below:]	(b2)	at (1,-1)	{};
\node [bv, label=above:]	(w2)	at (1,1)	{};
\path
\foreach \i/\j in {1/2}{
   	(w\i) edge [ev]   (b\j)
	%(b\i) edge [ev]  node [c, label=above:$\ell$] {} (w\j)
	(b\i) edge [ev]  node [c] {} (w\j)
	}
\foreach \i in {1,2}{
	(w\i)   edge 	[ev]				(b\i)
	(w\i)	edge [ev,bend left=30]	(b\i)
	(w\i)	edge [ev,bend right=30]	(b\i)
	}
\foreach \i in {w1,b1,w2,b2}{
   	%(\i) edge [e] (1)
	};
}
\end{tikzpicture}
}

\newcommand{\cvfl}{
\begin{tikzpicture}[x=2ex,y=2ex,baseline={([yshift=-.59ex]current bounding box.center)}] 
\scriptsize{
\node [v]	(1)	at (0,0)	{};
\node [vb, label=above:1]	(b1)	at (-1,1)	{};
\node [vb, label=below:2]	(w1)	at (-1,-1)	{};
\node [vb, label=below:7]	(b2)	at (1,-1)	{};
\node [vb, label=above:8]	(w2)	at (1,1)	{};
\path
\foreach \i/\j in {1/2}{
   	(w\i) edge [ev]   (b\j)
	(b\i) edge [ev]  node [c, label=above:$c$] {} (w\j)
	}
\foreach \i in {1,2}{
	(w\i)   edge 	[ev]				(b\i)
	(w\i)	edge [ev,bend left=30]	(b\i)
	(w\i)	edge [ev,bend right=30]	(b\i)
	}
\foreach \i in {w1,b1,w2,b2}{
   	(\i) edge [e] (1)
	};
}
\end{tikzpicture}
}

\newcommand{\cvft}{
\begin{tikzpicture}[scale=2,x=2ex,y=2ex,baseline={([yshift=-.59ex]current bounding box.center)}] 
\node [v]	(v)	at (0,0) 	{};
\node [vb]	(1)	at (-1,1)	{};
\node [vb]	(2)	at (-1,-1)	{};
\node [vb]	(3)	at (1,-1)	{};
\node [vb]	(4)	at (1,1)	{};
\path
\foreach \i in {1,2,3,4}{
    (\i) edge [e] (v)
    }
\foreach \i/\j in {1/2,2/1,3/4,4/3}{
   (\i)	edge [ev,bend left=15]	(\j)
   (\i)	edge [ev,bend left=40]	(\j)
   };
\end{tikzpicture}
}

\newcommand{\cvftneu}{
\begin{tikzpicture}[scale=2,x=2ex,y=2ex,baseline={([yshift=-.59ex]current bounding box.center)}] 
%\node [v]	(v)	at (0,0) 	{};
\node [wv]	(1)	at (-1,1)	{};
\node [bv]	(2)	at (-1,-1)	{};
\node [bv]	(3)	at (1,-1)	{};
\node [wv]	(4)	at (1,1)	{};
\path
%\foreach \i in {1,2,3,4}{
%    (\i) edge [e] (v)
%    }
\foreach \i/\j in {1/2,2/1,3/4,4/3}{
   (\i)	edge [ev,bend left=15]	(\j)
   (\i)	edge [ev,bend left=40]	(\j)
   };
\end{tikzpicture}
}

\newcommand{\cvfn}{
\begin{tikzpicture}[scale=2,x=2ex,y=2ex,baseline={([yshift=-.59ex]current bounding box.center)}] 
\scriptsize{
\node [v]	(1)	at (0,0)	{};
\node [vb, label=above:]	(b1)	at (-1,1)	{};
\node [vb, label=below:]	(w1)	at (-1,-1)	{};
\node [vb, label=below:]	(b2)	at (1,-1)	{};
\node [vb, label=above:]	(w2)	at (1,1)	{};
\path
\foreach \i/\j in {1/2,2/1}{
   	%(w\i) edge [ev]   (b\j)
   	%(w\i)	edge [ev,bend left=30]	(b\i)
   	(w\i) edge [ev,bend left=30]  (b\j)
   	(w\i) edge [ev,bend right=30] (b\j)
	%(b\i) edge [ev]  node [c, label=above:$\ell$] {} (w\j)
	}
\foreach \i in {1,2}{
	%(w\i)   edge 	[ev]				(b\i)
	(w\i)	edge [ev,bend left=30]  (b\i)
	(w\i)	edge [ev,bend right=30]	(b\i)
	}
\foreach \i in {w1,b1,w2,b2}{
   	(\i) edge [e] (1)
	};
}
\end{tikzpicture}
}

\newcommand{\cvfnneu}{
\begin{tikzpicture}[scale=2,x=2ex,y=2ex,baseline={([yshift=-.59ex]current bounding box.center)}] 
\scriptsize{
%\node [v]	(1)	at (0,0)	{};
\node [wv, label=above:]	(b1)	at (-1,1)	{};
\node [bv, label=below:]	(w1)	at (-1,-1)	{};
\node [wv, label=below:]	(b2)	at (1,-1)	{};
\node [bv, label=above:]	(w2)	at (1,1)	{};
\path
\foreach \i/\j in {1/2,2/1}{
   	%(w\i) edge [ev]   (b\j)
   	%(w\i)	edge [ev,bend left=30]	(b\i)
   	(w\i) edge [ev,bend left=30]  (b\j)
   	(w\i) edge [ev,bend right=30] (b\j)
	%(b\i) edge [ev]  node [c, label=above:$\ell$] {} (w\j)
	}
\foreach \i in {1,2}{
	%(w\i)   edge 	[ev]				(b\i)
	(w\i)	edge [ev,bend left=30]  (b\i)
	(w\i)	edge [ev,bend right=30]	(b\i)
	}
\foreach \i in {w1,b1,w2,b2}{
   %	(\i) edge [e] (1)
	};
}
\end{tikzpicture}
}

\newcommand{\cvfsvg}{
\begin{tikzpicture}[x=1ex,y=1ex,baseline={([yshift=-.59ex]current bounding box.center)}] 
\scriptsize{
%\node [v]	(0)	at (0,0)	{};
\foreach \i in {72,144,216,288,360}{
\begin{scope}[rotate=\i]
\node [vb]	(\i)	at (0,1.6)	{};
\end{scope}
}
\path
\foreach \i in {72,144,216,288,360}{
    \foreach \j in {72,144,216,288,360}{
   	    (\i) edge [ev]  (\j)
	    }
%     }
% \foreach \i in {72,144,216,288,360}{
%   	(\i) edge [e] (0)
	};
}
\end{tikzpicture}
}

\newcommand{\cvfs}{
\begin{tikzpicture}[scale=2,x=2ex,y=2ex,baseline={([yshift=-.59ex]current bounding box.center)}] 
\scriptsize{
\node [v]	(0)	at (0,0)	{};
\foreach \i in {72,144,216,288,360}{
\begin{scope}[rotate=\i]
\node [vb]	(\i)	at (0,1.6)	{};
\end{scope}
}
\path
\foreach \i in {72,144,216,288,360}{
    \foreach \j in {72,144,216,288,360}{
   	    (\i) edge [ev]  (\j)
	    }
    }
\foreach \i in {72,144,216,288,360}{
  	(\i) edge [e] (0)
	};
}
\end{tikzpicture}
}

\newcommand{\cvfsneu}{
\begin{tikzpicture}[scale=2,x=2ex,y=2ex,baseline={([yshift=-.59ex]current bounding box.center)}] 
\scriptsize{
%\node [v]	(0)	at (0,0)	{};
\foreach \i in {72,144,216,288,360}{
\begin{scope}[rotate=\i]
\node [bv]	(\i)	at (0,1.6)	{};
\end{scope}
}
\path
\foreach \i in {72,144,216,288,360}{
    \foreach \j in {72,144,216,288,360}{
   	    (\i) edge [ev]  (\j)
	    }
    }
\foreach \i in {72,144,216,288,360}{
  	%(\i) edge [e] (0)
	};
}
\end{tikzpicture}
}


\newcommand{\cvftl}{
\begin{tikzpicture}[x=2ex,y=2ex,baseline={([yshift=-.59ex]current bounding box.center)}] 
\scriptsize{
\node [v]	(v)	at (0,0) 	{};
\node [vb, label=above:1]	(1)	at (-1,1)	{};
\node [vb, label=below:2]	(2)	at (-1,-1)	{};
\node [vb, label=below:7]	(3)	at (1,-1)	{};
\node [vb, label=above:8]	(4)	at (1,1)	{};
\path
\foreach \i in {1,2,3,4}{
    (\i) edge [e] (v)
    }
\foreach \i/\j in {1/2,2/1,3/4,4/3}{
   (\i)	edge [ev,bend left=15]	(\j)
   (\i)	edge [ev,bend left=40]	(\j)
   };
}
\end{tikzpicture}
}

\newcommand{\cfishl}{
\begin{tikzpicture}[x=2ex,y=2ex,baseline={([yshift=-.59ex]current bounding box.center)}] 
\scriptsize{
\node [v]	(1)	at (0,0)	{};
\node [v]	(2)	at (4,0)	{};
\node [vb, label=above:1]	(b1)	at (-1,1)	{};
\node [vb, label=below:2]	(w1)	at (-1,-1)	{};
\node [vb, label=below:3]	(b2)	at (1,-1)	{};
\node [vb, label=above:4]	(w2)	at (1,1)	{};
\node [vb, label=above:5]	(b3)	at (3,1)	{};
\node [vb, label=below:6]	(w3)	at (3,-1)	{};
\node [vb, label=below:7]	(b4)	at (5,-1)	{};
\node [vb, label=above:8]	(w4)	at (5,1)	{};
\path
\foreach \i/\j in {1/2}{
   	(w\i) edge [ev]   (b\j)
	(b\i) edge [ev]  node [c, label=above:$c_1$] {} (w\j)
	}
\foreach \i/\j in {3/4}{
   	(w\i) edge [ev]   (b\j)
	(b\i) edge [ev]  node [c, label=above:$c_2$] {} (w\j)
	}
\foreach \i in {1,2,3,4}{
	(w\i) edge 	[ev]				(b\i)
	(w\i)	edge [ev,bend left=30]	(b\i)
	(w\i)	edge [ev,bend right=30]	(b\i)
	}
\foreach \i in {w1,b1,w2,b2}{
   	(\i) edge [e] (1)
	}
\foreach \i in {w3,b3,w4,b4}{
   	(\i) edge [e] (2)
	}	
\foreach \i/\j in {w2/b3,w3/b2}{
   	(\i) edge [es] (\j)
	};
}
\end{tikzpicture}
}

\newcommand{\cfishlc}{
\begin{tikzpicture}[x=2ex,y=2ex,baseline={([yshift=-.59ex]current bounding box.center)}] 
\scriptsize{
\node [v]	(1)	at (0,0)	{};
\node [v]	(2)	at (4,0)	{};
\node [vb, label=above:1]	(b1)	at (-1,1)	{};
\node [vb, label=below:2]	(w1)	at (-1,-1)	{};
\node [vb, label=below:3]	(b2)	at (1,-1)	{};
\node [vb, label=above:4]	(w2)	at (1,1)	{};
\node [vb, label=above:5]	(b3)	at (3,1)	{};
\node [vb, label=below:6]	(w3)	at (3,-1)	{};
\node [vb, label=below:7]	(b4)	at (5,-1)	{};
\node [vb, label=above:8]	(w4)	at (5,1)	{};
\path
\foreach \i/\j in {1/2,3/4}{
   	(w\i) edge [ev]   (b\j)
	(b\i) edge [ev]  node [c, label=above:$c$] {} (w\j)
    }
\foreach \i in {1,2,3,4}{
	(w\i) edge 	[ev]				(b\i)
	(w\i)	edge [ev,bend left=30]	(b\i)
	(w\i)	edge [ev,bend right=30]	(b\i)
	}
\foreach \i in {w1,b1,w2,b2}{
   	(\i) edge [e] (1)
	}
\foreach \i in {w3,b3,w4,b4}{
   	(\i) edge [e] (2)
	}	
\foreach \i/\j in {w2/b3,w3/b2}{
   	(\i) edge [es] (\j)
	};
}
\end{tikzpicture}
}

\newcommand{\cfish}{
\begin{tikzpicture}[x=2ex,y=2ex,baseline={([yshift=-.59ex]current bounding box.center)}] 
\scriptsize{
\node [v]	(1)	at (0,0)	{};
\node [v]	(2)	at (4,0)	{};
\node [vb]	(w1)	at (-1,-1)	{};
\node [vb]	(b1)	at (-1,1)	{};
\node [vb]	(w2)	at (1,1)	{};
\node [vb]	(b2)	at (1,-1)	{};
\node [vb]	(w3)	at (3,-1)	{};
\node [vb]	(b3)	at (3,1)	{};
\node [vb]	(w4)	at (5,1)	{};
\node [vb]	(b4)	at (5,-1)	{};
\path
\foreach \i/\j in {1/2,3/4}{
   	(w\i) edge [ev]   (b\j)
	(b\i) edge [ev]  node [c] {} (w\j)
	}
\foreach \i in {1,2,3,4}{
	(w\i) edge 	[ev]				(b\i)
	(w\i)	edge [ev,bend left=30]	(b\i)
	(w\i)	edge [ev,bend right=30]	(b\i)
	}
\foreach \i in {w1,b1,w2,b2}{
   	(\i) edge [e] (1)
	}
\foreach \i in {w3,b3,w4,b4}{
   	(\i) edge [e] (2)
	}	
\foreach \i/\j in {w2/b3,w3/b2}{
   	(\i) edge [es] (\j)
	};
}
\end{tikzpicture}
}

\newcommand{\cfisha}{
\begin{tikzpicture}[x=2ex,y=2ex,baseline={([yshift=-.59ex]current bounding box.center)}] 
\scriptsize{
\node [v]	(1)	at (0,0)	{};
\node [v]	(2)	at (4,0)	{};
\node [vb]	(w1)	at (-1,-1)	{};
\node [vb]	(b1)	at (-1,1)	{};
\node [vb]	(w2)	at (1,1)	{};
\node [vb]	(b2)	at (1,-1)	{};
\node [vb]	(w3)	at (3,-1)	{};
\node [vb]	(b3)	at (3,1)	{};
\node [vb]	(w4)	at (5,1)	{};
\node [vb]	(b4)	at (5,-1)	{};
\path
\foreach \i/\j in {1/2,3/4}{
   	(w\i) edge [ev]   (b\j)
	(b\i) edge [ev]  node [c] {} (w\j)
	}
\foreach \i in {1,2,3,4}{
	(w\i) edge 	[ev]				(b\i)
	(w\i)	edge [ev,bend left=30]	(b\i)
	(w\i)	edge [ev,bend right=30]	(b\i)
	}
\foreach \i in {w1,b1,w2,b2}{
   	(\i) edge [e] (1)
	}
\foreach \i in {w3,b3,w4,b4}{
   	(\i) edge [e] (2)
	}	
\foreach \i/\j in {w3/b2}{
   	(\i) edge [es] (\j)
	};
}
\end{tikzpicture}
}

\newcommand{\cfishb}{
\begin{tikzpicture}[x=2ex,y=2ex,baseline={([yshift=-.59ex]current bounding box.center)}] 
\scriptsize{
\node [v]	(1)	at (0,0)	{};
\node [v]	(2)	at (4,0)	{};
\node [vb]	(w1)	at (-1,-1)	{};
\node [vb]	(b1)	at (-1,1)	{};
\node [vb]	(w2)	at (1,1)	{};
\node [vb]	(b2)	at (1,-1)	{};
\node [vb]	(w3)	at (3,-1)	{};
\node [vb]	(b3)	at (3,1)	{};
\node [vb]	(w4)	at (5,1)	{};
\node [vb]	(b4)	at (5,-1)	{};
\path
\foreach \i/\j in {1/2,3/4}{
   	(w\i) edge [ev]   (b\j)
	(b\i) edge [ev]  node [c] {} (w\j)
	}
\foreach \i in {1,2,3,4}{
	(w\i) edge 	[ev]				(b\i)
	(w\i)	edge [ev,bend left=30]	(b\i)
	(w\i)	edge [ev,bend right=30]	(b\i)
	}
\foreach \i in {w1,b1,w2,b2}{
   	(\i) edge [e] (1)
	}
\foreach \i in {w3,b3,w4,b4}{
   	(\i) edge [e] (2)
	}	
\foreach \i/\j in {w2/b3}{
   	(\i) edge [es] (\j)
	};
}
\end{tikzpicture}
}

\newcommand{\cfishc}{
\begin{tikzpicture}[x=2ex,y=2ex,baseline={([yshift=-.59ex]current bounding box.center)}] 
\scriptsize{
\node [v]	(1)	at (0,0)	{};
\node [v]	(2)	at (4,0)	{};
\node [vb]	(w1)	at (-1,-1)	{};
\node [vb]	(b1)	at (-1,1)	{};
\node [vb]	(w2)	at (1,1)	{};
\node [vb]	(b2)	at (1,-1)	{};
\node [vb]	(w3)	at (3,-1)	{};
\node [vb]	(b3)	at (3,1)	{};
\node [vb]	(w4)	at (5,1)	{};
\node [vb]	(b4)	at (5,-1)	{};
\path
\foreach \i/\j in {1/2,3/4}{
   	(w\i) edge [ev]   (b\j)
	(b\i) edge [ev]  node [c] {} (w\j)
	}
\foreach \i in {1,2,3,4}{
	(w\i) edge 	[ev]				(b\i)
	(w\i)	edge [ev,bend left=30]	(b\i)
	(w\i)	edge [ev,bend right=30]	(b\i)
	}
\foreach \i in {w1,b1,w2,b2}{
   	(\i) edge [e] (1)
	}
\foreach \i in {w3,b3,w4,b4}{
   	(\i) edge [e] (2)
	};
}
\end{tikzpicture}
}


\newcommand{\cvsla}{
\begin{tikzpicture}[x=2ex,y=2ex,baseline={([yshift=0ex]current bounding box.center)}]
\scriptsize{
\node [v]	(1)	at (0,0)	{};
\begin{scope}[rotate=120]
\node [vb, label=left:1]		(b1)	at (.7,1.2)	{};
\node [vb, label=below:2]		(w1)	at (-.7,1.2)	{};
\end{scope}
\begin{scope}[rotate=240]
\node [vb, label=below:7]		(b2)	at (.7,1.2)	{};
\node [vb, label=right:8]		(w2)	at (-.7,1.2)	{};
\end{scope}
\begin{scope}[rotate=0]
\node [vb, label=right:5]		(b3)	at (.7,1.2)	{};
\node [vb, label=left:4]		(w3)	at (-.7,1.2)	{};
\end{scope}	
\path
(w1) edge [ev]  node [c, label=below:$c$] {} (b2)
\foreach \i/\j in {2/3,3/1}{
   	(w\i) edge [ev]   (b\j)
	}
\foreach \i in {1,2,3}{
	(w\i) edge 	[ev]				(b\i)
	(w\i)	edge [ev,bend left=30]	(b\i)
	(w\i)	edge [ev,bend right=30]	(b\i)
	}
\foreach \i in {w1,b1,w2,b2,w3,b3}{
   	(\i) edge [e] (1)
	}
(w3) edge [es, bend left=90] (b3);
}
\end{tikzpicture}
}

\newcommand{\cvslb}{
\begin{tikzpicture}[x=2ex,y=2ex,baseline={([yshift=-1.2ex]current bounding box.center)}]
\scriptsize{
\node [v]	(1)	at (0,0)	{};
\begin{scope}[rotate=60]
\node [vb, label=above:1]		(b1)	at (.7,1.2)	{};
\node [vb, label=left:2]		(w1)	at (-.7,1.2)	{};
\end{scope}
\begin{scope}[rotate=180]
\node [vb, label=left:3]		(b2)	at (.7,1.2)	{};
\node [vb, label=right:6]		(w2)	at (-.7,1.2)	{};
\end{scope}
\begin{scope}[rotate=300]
\node [vb, label=right:7]		(b3)	at (.7,1.2)	{};
\node [vb, label=above:8]		(w3)	at (-.7,1.2)	{};
\end{scope}	
\path
(b1) edge [ev]  node [c, label=above:$c$] {} (w3)
\foreach \i/\j in {1/2,2/3}{
   	(w\i) edge [ev]   (b\j)
	}
\foreach \i in {1,2,3}{
	(w\i) edge 	[ev]				node 	{}	(b\i)
	(w\i)	edge [ev,bend left=30]	node 	{}	(b\i)
	(w\i)	edge [ev,bend right=30]	node 	{}	(b\i)
	}
\foreach \i in {w1,b1,w2,b2,w3,b3}{
   	(\i) edge [e] (1)
	}
(w2) edge [es, bend left=90] (b2);
}
\end{tikzpicture}
}

\newcommand{\cvslc}{
\begin{tikzpicture}[x=2ex,y=2ex,baseline={([yshift=-.59ex]current bounding box.center)}]
\scriptsize{
\node [v]	(1)	at (0,0)	{};
\begin{scope}[rotate=90]
\node [vb, label=left:1]		(b1)	at (.7,1.2)	{};
\node [vb, label=left:2]		(w1)	at (-.7,1.2)	{};
\end{scope}
\begin{scope}[rotate=210]
\node [vb, label=below:5]		(b2)	at (.7,1.2)	{};
\node [vb, label=right:8]		(w3)	at (-.7,1.2)	{};
\end{scope}
\begin{scope}[rotate=330]
\node [vb, label=right:7]		(b3)	at (.7,1.2)	{};
\node [vb, label=above:4]		(w2)	at (-.7,1.2)	{};
\end{scope}	
\path
(b1) edge [ev]  node [c, label=150:$c_1$] {} (w2)
(w2) edge [ev]  node [c, label=30:$c_2$] {} (b3)
\foreach \i/\j in {1/1,1/2,3/2,3/3}{
   	(w\i) edge [ev]   (b\j)
	}
\foreach \i in {1,2,3}{
	(w\i)	edge [ev,bend left=30]	node 	{}	(b\i)
	(w\i)	edge [ev,bend right=30]	node 	{}	(b\i)
	}
\foreach \i in {w1,b1,w2,b2,w3,b3}{
   	(\i) edge [e] (1)
	}
(w2) edge [es, bend left=140] (b2);
}
\end{tikzpicture}
}

\newcommand{\cvsld}{
\begin{tikzpicture}[x=2ex,y=2ex,baseline={([yshift=-.59ex]current bounding box.center)}]
\scriptsize{
\node [v]	(1)	at (0,0)	{};
\begin{scope}[rotate=90]
\node [vb, label=left:1]		(b1)	at (.7,1.2)	{};
\node [vb, label=left:2]		(w1)	at (-.7,1.2)	{};
\end{scope}
\begin{scope}[rotate=210]
\node [vb, label=below:6]		(b2)	at (.7,1.2)	{};
\node [vb, label=right:8]		(w3)	at (-.7,1.2)	{};
\end{scope}
\begin{scope}[rotate=330]
\node [vb, label=right:7]		(b3)	at (.7,1.2)	{};
\node [vb, label=above:3]		(w2)	at (-.7,1.2)	{};
\end{scope}	
\path
(b1) edge [ev]  node [c, label=150:$c_1$] {} (w2)
(w2) edge [ev]  node [c, label=30:$c_2$] {} (b3)
\foreach \i/\j in {1/1,1/2,3/2,3/3}{
   	(w\i) edge [ev]   (b\j)
	}
\foreach \i in {1,2,3}{
	(w\i)	edge [ev,bend left=30]	node 	{}	(b\i)
	(w\i)	edge [ev,bend right=30]	node 	{}	(b\i)
	}
\foreach \i in {w1,b1,w2,b2,w3,b3}{
   	(\i) edge [e] (1)
	}
(w2) edge [es, bend left=140] (b2);
}
\end{tikzpicture}
}

\newcommand{\cvsd}{
\begin{tikzpicture}[x=2ex,y=2ex,baseline={([yshift=-.59ex]current bounding box.center)}]
\scriptsize{
\node [v]	(1)	at (0,0)	{};
\begin{scope}[rotate=90]
\node [vb]		(b1)	at (.7,1.2)	{};
\node [vb]		(w1)	at (-.7,1.2)	{};
\end{scope}
\begin{scope}[rotate=210]
\node [vb]		(b2)	at (.7,1.2)	{};
\node [vb]		(w3)	at (-.7,1.2)	{};
\end{scope}
\begin{scope}[rotate=330]
\node [vb]		(b3)	at (.7,1.2)	{};
\node [vb]		(w2)	at (-.7,1.2)	{};
\end{scope}	
\path
% (b1) edge [ev]  node [c, label=150:$c_1$] {} (w2)
% (w2) edge [ev]  node [c, label=30:$c_2$] {} (b3)
\foreach \i/\j in {1/1,1/2,2/1,2/3,3/2,3/3}{
   	(w\i) edge [ev]   (b\j)
	}
\foreach \i in {1,2,3}{
	(w\i)	edge [ev,bend left=30]	node 	{}	(b\i)
	(w\i)	edge [ev,bend right=30]	node 	{}	(b\i)
	}
\foreach \i in {w1,b1,w2,b2,w3,b3}{
   	(\i) edge [e] (1)
	}
(w2) edge [es, bend left=140] (b2);
}
\end{tikzpicture}
}
